Discrete Minds in a Continuous World: Do Language Models Know Time Passes?

While Large Language Models (LLMs) excel at temporal reasoning tasks like event ordering and duration estimation, their ability to perceive the actual passage of time remains unexplored. We investigate whether LLMs perceive the passage of time and adapt their decision-making accordingly through three complementary experiments. First, we introduce the Token-Time Hypothesis, positing that LLMs can map discrete token counts to continuous wall-clock time, and validate this through a dialogue duration judgment task. Second, we demonstrate that LLMs could use this awareness to adapt their response length while maintaining accuracy when users express urgency in question answering tasks. Finally, we develop BombRush, an interactive navigation challenge that examines how LLMs modify behavior under progressive time pressure in dynamic environments. Our findings indicate that LLMs possess certain awareness of time passage, enabling them to bridge discrete linguistic tokens and continuous physical time, though this capability varies with model size and reasoning abilities. This work establishes a theoretical foundation for enhancing temporal awareness in LLMs for time-sensitive applications.

==> Figures/s_bombrush_static_appedix.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{Figures/br_appendix_7.pdf}
    \caption{Token usage dynamics across all 7 Bomb Rush scenarios. Each row corresponds to one task variant, grouped into three main settings: (a) Treasure Hunt (S1), (b–e) Static Bomb with 4 prompt variants (S2), and (f–g) Moving Bomb with and without active detection (S3). For each model, the \textcolor{orange}{orange curve} indicates the average number of tokens generated per step, with shaded areas representing standard deviation. The \textcolor{ForestGreen}{green line} (where applicable) shows the remaining time as the task progresses. This visualization highlights how different models adapt their token usage under varying temporal constraints and scenario complexities.
    }
    \label{fig:bomb_rush_7_appendix}
\end{figure*}

==> Figures/s_moving_bomb_prompt.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{Figures/moving_bomb_prompt.pdf}
    \caption{System prompt used in the Moving Bomb scenario of the Bomb Rush task.}
    \label{fig:moving_bomb_prompt}
\end{figure*}

==> Table/bomb_static_result.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{llcccccc}
\hline
\textbf{Model} & \textbf{Settings} & \textbf{\begin{tabular}[c]{@{}c@{}}\% \\ Success\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}\% \\ Over Steps\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}\% \\ Time Out\end{tabular}} & \textbf{\# Steps} & \textbf{\begin{tabular}[c]{@{}c@{}}Navigation \\ Accuracy ↑\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Time \\ Efficiency ↑\end{tabular}} \\ \hline
\multirow{9}{*}{\textbf{Llama-3.3-70B}} & S1: Treasure Hunt & 83\% & 17\% & 0\% & 9.5 & 75.4\% & - \\
 & S2: Bomb Rush & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
 & \hspace{1em}Static Bomb-Baseline & 76\% & 0\% & 24\% & 7.6 & 71.8\% & 31.5\% \\
 & \hspace{1em}Static Bomb-Hint & 82\% & 0\% & 18\% & 7.7 & 75.5\% & 35.1\% \\
 & \hspace{1em}Static Bomb-Hunry & 76\% & 0\% & 24\% & 8.1 & 70.4\% & 31.8\% \\
 & \hspace{1em}Static Bomb-Hint\&Hurry & 75\% & 0\% & 25\% & 8.3 & 67.0\% & 32.6\% \\
 & S3: Bomb Rush Hard & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
 & \hspace{1em}Moving Bomb Baseline & 69\% & 0\% & 31\% & 7.7 & - & 28.5\% \\
 & \hspace{1em}Moving Bomb w/ Detection & 49\% & 0\% & 51\% & 9.9 & - & 15.3\% \\ \hline
\multirow{9}{*}{\textbf{Qwen2.5-72B}} & S1: Treasure Hunt & 89\% & 11\% & 0\% & 9.9 & 75.0\% & - \\
 & S2: Bomb Rush & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
 & \hspace{1em}Static Bomb-Baseline & 87\% & 13\% & 0\% & 9.5 & 75.8\% & 72.6\% \\
 & \hspace{1em}Static Bomb-Hint & 90\% & 10\% & 0\% & 9.9 & 73.9\% & 74.0\% \\
 & \hspace{1em}Static Bomb-Hunry & 87\% & 13\% & 0\% & 9.8 & 74.4\% & 72.3\% \\
 & \hspace{1em}Static Bomb-Hint\&Hurry & 90\% & 10\% & 0\% & 9.8 & 75.6\% & 74.3\% \\
 & S3: Bomb Rush Hard & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
 & \hspace{1em}Moving Bomb Baseline & 86\% & 14\% & 0\% & 12.0 & - & 67.9\% \\
 & \hspace{1em}Moving Bomb w/ Detection & 63\% & 37\% & 0\% & 18.7 & - & 45.8\% \\ \hline
\multirow{9}{*}{\textbf{DS-R1-Llama-70B}} & S1: Treasure Hunt & 67\% & 33\% & 0\% & 11.7 & 61.5\% & - \\
 & S2: Bomb Rush &  &  &  &  &  &  \\
 & \hspace{1em}Static Bomb-Baseline & 80\% & 20\% & 0\% & 10.1 & 71.5\% & 65.4\% \\
 & \hspace{1em}Static Bomb-Hint & 72\% & 28\% & 0\% & 11.0 & 66.2\% & 59.4\% \\
 & \hspace{1em}Static Bomb-Hunry & 72\% & 28\% & 0\% & 11.4 & 64.4\% & 57.9\% \\
 & \hspace{1em}Static Bomb-Hint\&Hurry & 70\% & 30\% & 0\% & 11.6 & 62.8\% & 57.2\% \\
 & S3: Bomb Rush Hard & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
 & \hspace{1em}Moving Bomb Baseline & 74\% & 26\% & 0\% & 14.4 & - & 58.7\% \\
 & \hspace{1em}Moving Bomb w/ Detection & 79\% & 21\% & 0\% & 15.8 & - & 53.5\% \\ \hline
\multirow{9}{*}{\textbf{QwQ-32B}} & S1: Treasure Hunt & 97\% & 3\% & 0\% & 7.8 & 91.7\% & - \\
 & S2: Bomb Rush & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
 & \hspace{1em}Static Bomb-Baseline & 83\% & 0\% & 17\% & 6.7 & 82.0\% & 40.6\% \\
 & \hspace{1em}Static Bomb-Hint & 86\% & 0\% & 14\% & 6.5 & 85.1\% & 40.9\% \\
 & \hspace{1em}Static Bomb-Hunry & 84\% & 0\% & 16\% & 6.5 & 83.2\% & 41.9\% \\
 & \hspace{1em}Static Bomb-Hint\&Hurry & 85\% & 0\% & 15\% & 6.2 & 83.7\% & 42.1\% \\
 & S3: Bomb Rush Hard & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
 & \hspace{1em}Moving Bomb Baseline & 85\% & 0\% & 15\% & 6.9 & - & 38.9\% \\
 & \hspace{1em}Moving Bomb w/ Detection & 63\% & 0\% & 37\% & 9.0 & - & 23.5\% \\ \hline
\end{tabular}%
}
\caption{Evaluation results on the S1 Treasure Hunt, S2 Bomb Rush and S3 Bomb Rush Hard tasks.}
\label{tab:static_bomb_result}
\end{table*}

% \begin{tabular}{@{}llcccccccc@{}}
% \toprule
% \textbf{Model} & \textbf{Settings} & \multicolumn{1}{l}{\textbf{\% Success}} & \multicolumn{1}{l}{\textbf{\% Over Steps}} & \multicolumn{1}{l}{\textbf{\% Time Out}} & \multicolumn{1}{l}{\textbf{\# Steps}} & \multicolumn{1}{l}{\textbf{\# Think Tokens}} & \multicolumn{1}{l}{\textbf{\# Solution Tokens}} & \multicolumn{1}{l}{\textbf{Navigation Accuracy ↑}} & \multicolumn{1}{l}{\textbf{Time Efficiency ↑}} \\ \midrule
% \multirow{5}{*}{\textbf{Llama-3.3-70B}} & Static Treasure & 83\% & 17\% & 0\% & 9.5 & - & 235 & 75.4\% & 83.0\% \\
%  & Static Bomb & 76\% & 0\% & 24\% & 7.6 & - & 278 & 71.8\% & 31.5\% \\
%  & SB-Hint & 82\% & 0\% & 18\% & 7.7 & - & 257 & 75.5\% & 35.1\% \\
%  & SB-Hurry & 76\% & 0\% & 24\% & 8.1 & - & 258 & 70.4\% & 31.8\% \\
%  & SB-Hint+Hurry & 75\% & 0\% & 25\% & 8.3 & - & 246 & 67.0\% & 32.6\% \\ \midrule
% \multirow{5}{*}{\textbf{Qwen2.5-72B}} & Static Treasure & 89\% & 11\% & 0\% & 9.9 & - & 57 & 75.0\% & 89.0\% \\
%  & Static Bomb & 87\% & 13\% & 0\% & 9.5 & - & 60 & 75.8\% & 72.6\% \\
%  & SB-Hint & 90\% & 10\% & 0\% & 9.9 & - & 58 & 73.9\% & 74.0\% \\
%  & SB-Hurry & 87\% & 13\% & 0\% & 9.8 & - & 59 & 74.4\% & 72.3\% \\
%  & SB-Hint+Hurry & 90\% & 11\% & 0\% & 9.8 & - & 58 & 75.6\% & 74.3\% \\ \midrule
% \multirow{5}{*}{\textbf{DS-Llama-70B}} & Static Treasure & 67\% & 33\% & 0\% & 11.7 & 516 & 64 & 61.5\% & 67.0\% \\
%  & Static Bomb & 80\% & 20\% & 0\% & 10.1 & 574 & 72 & 71.5\% & 65.4\% \\
%  & SB-Hint & 72\% & 28\% & 0\% & 11.0 & 565 & 75 & 66.2\% & 59.4\% \\
%  & SB-Hurry & 72\% & 28\% & 0\% & 11.4 & 609 & 72 & 64.4\% & 57.9\% \\
%  & SB-Hint+Hurry & 70\% & 31\% & 0\% & 11.6 & 547 & 66 & 62.8\% & 57.2\% \\ \midrule
% \multirow{5}{*}{\textbf{QwQ-32B}} & Static Treasure & 97\% & 3\% & 0\% & 7.8 & 2391 & 80 & 91.7\% & 97.0\% \\
%  & Static Bomb & 83\% & 0\% & 17\% & 6.7 & 2575 & 89 & 82.0\% & 40.6\% \\
%  & SB-Hint & 86\% & 0\% & 14\% & 6.5 & 2622 & 90 & 85.1\% & 40.9\% \\
%  & SB-Hurry & 84\% & 0\% & 16\% & 6.5 & 2610 & 88 & 83.2\% & 41.9\% \\
%  & SB-Hint+Hurry & 85\% & 0\% & 15\% & 6.2 & 2732 & 87 & 83.7\% & 42.1\% \\ \bottomrule
% \end{tabular}%

% \begin{tabular}{@{}llcccccccc@{}}
% \toprule
% \textbf{Model} & \textbf{Settings} & \textbf{\begin{tabular}[c]{@{}c@{}}\% \\ Success\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}\% \\ Over Steps\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}\% \\ Time Out\end{tabular}} & \textbf{\# Steps} & \textbf{\begin{tabular}[c]{@{}c@{}}\# Think \\ Tokens\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}\# Solution \\ Tokens\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Navigation \\ Accuracy ↑\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Time \\ Efficiency ↑\end{tabular}} \\ \midrule
% \multirow{7}{*}{\textbf{Llama-3.3-70B}} & Static Treasure & 83\% & 17\% & 0\% & 9.5 & - & 235 & 75.4\% & 83.0\% \\
%  & Static Bomb & 76\% & 0\% & 24\% & 7.6 & - & 278 & 71.8\% & 31.5\% \\
%  & \hspace{1em}SB-Hint & 82\% & 0\% & 18\% & 7.7 & - & 257 & 75.5\% & 35.1\% \\
%  & \hspace{1em}SB-Hurry & 76\% & 0\% & 24\% & 8.1 & - & 258 & 70.4\% & 31.8\% \\
%  & \hspace{1em}SB-Hint+Hurry & 75\% & 0\% & 25\% & 8.3 & - & 246 & 67.0\% & 32.6\% \\
%  & Moving & 69\% & 0\% & 31\% & 7.7 & - & 279 & - & 28.5\% \\
%  & Moving wd & 49\% & 0\% & 51\% & 9.9 & - & 258 & - & 15.3\% \\ \midrule
% \multirow{7}{*}{\textbf{Qwen2.5-72B}} & Static Treasure & 89\% & 11\% & 0\% & 9.9 & - & 57 & 75.0\% & 89.0\% \\
%  & Static Bomb & 87\% & 13\% & 0\% & 9.5 & - & 60 & 75.8\% & 72.6\% \\
%  & \hspace{1em}SB-Hint & 90\% & 10\% & 0\% & 9.9 & - & 58 & 73.9\% & 74.0\% \\
%  & \hspace{1em}SB-Hurry & 87\% & 13\% & 0\% & 9.8 & - & 59 & 74.4\% & 72.3\% \\
%  & \hspace{1em}SB-Hint+Hurry & 90\% & 10\% & 0\% & 9.8 & - & 58 & 75.6\% & 74.3\% \\
%  & Moving & 86\% & 14\% & 0\% & 12.0 & - & 67 & - & 67.9\% \\
%  & Moving wd & 63\% & 37\% & 0\% & 18.7 & - & 64 & - & 45.8\% \\ \midrule
% \multirow{7}{*}{\textbf{DS-R1-Llama-70B}} & Static Treasure & 67\% & 33\% & 0\% & 11.7 & 516 & 64 & 61.5\% & 67.0\% \\
%  & Static Bomb & 80\% & 20\% & 0\% & 10.1 & 574 & 72 & 71.5\% & 65.4\% \\
%  & \hspace{1em}SB-Hint & 72\% & 28\% & 0\% & 11.0 & 565 & 75 & 66.2\% & 59.4\% \\
%  & \hspace{1em}SB-Hurry & 72\% & 28\% & 0\% & 11.4 & 609 & 72 & 64.4\% & 57.9\% \\
%  & \hspace{1em}SB-Hint+Hurry & 70\% & 30\% & 0\% & 11.6 & 547 & 66 & 62.8\% & 57.2\% \\
%  & Moving & 74\% & 26\% & 0\% & 14.4 & 547 & 65 & - & 58.7\% \\
%  & Moving wd & 79\% & 21\% & 0\% & 15.8 & 612 & 70 & - & 53.5\% \\ \midrule
% \multirow{7}{*}{\textbf{QwQ-32B}} & Static Treasure & 97\% & 3\% & 0\% & 7.8 & 2391 & 80 & 91.7\% & 97.0\% \\
%  & Static Bomb & 83\% & 0\% & 17\% & 6.7 & 2575 & 89 & 82.0\% & 40.6\% \\
%  & \hspace{1em}SB-Hint & 86\% & 0\% & 14\% & 6.5 & 2622 & 90 & 85.1\% & 40.9\% \\
%  & \hspace{1em}SB-Hurry & 84\% & 0\% & 16\% & 6.5 & 2610 & 88 & 83.2\% & 41.9\% \\
%  & \hspace{1em}SB-Hint+Hurry & 85\% & 0\% & 15\% & 6.2 & 2732 & 87 & 83.7\% & 42.1\% \\
%  & Moving & 85\% & 0\% & 15\% & 6.9 & 2480 & 90 & - & 38.9\% \\
%  & Moving wd & 63\% & 0\% & 37\% & 9.0 & 2495 & 86 & - & 23.5\% \\ \bottomrule
% \end{tabular}%

==> Table/bombrush_compare.tex <==
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lccc@{}}
\toprule
\textbf{Feature} & \multicolumn{1}{l}{\textbf{Time Pressure}} & \multicolumn{1}{l}{\textbf{Moving Target}} & \multicolumn{1}{l}{\textbf{Signal Source}} \\ \midrule
T1: Treasure Hunt & \textcolor{blue}{\ding{55}} & {\ding{55}} & Passive \\
T2: Static Bomb & \textcolor{green}{\ding{51}} & {\ding{55}} & Passive \\
T3: Moving Bomb & \textcolor{orange}{\ding{51}} & {\ding{51}} & Passive \\
T4: Moving Bomb w/ D & \textcolor{red}{\ding{51}} & {\ding{51}} & Proactive \\ \bottomrule
\end{tabular}%
}
\caption{Each subtask is characterized along three key dimensions: the presence of time pressure, whether the target (treasure or bomb) moves, and how signal information is acquired—either passively emitted or requiring proactive detection. Time pressure is visually encoded: \textcolor{orange}{\ding{51}} indicates moderate urgency, \textcolor{red}{\ding{51}} indicates high urgency, and \textcolor{blue}{\ding{55}} denotes no time pressure. These task variants are designed to progressively increase temporal and strategic complexity, enabling analysis of LLM decision-making under dynamic constraints.}
\label{tab:bombrush_compare}
\end{table}

==> sections/Backups.tex <==

\section{Full Experimental Settings of Bomb Rush}
\paragraph{S1: Treasure Hunt.}
In this baseline setting, the agent navigates to a stationary treasure with no time constraints. The treasure emits directional signals indicating distance and direction. This setting evaluates the model’s fundamental spatial reasoning capabilities without temporal pressure. The corresponding system prompt is shown in~\Cref{fig:treasure_prompt}.
\input{Figures/s_treasure_prompt}

\paragraph{S2: Bomb Rush.}
The agent must locate a stationary bomb that detonates after a fixed countdown. Like S1, the bomb emits directional signals, but now the agent must operate under time pressure. We define 4 variants under this setting based on how temporal information is communicated:

\begin{itemize}
\item \textbf{Static Bomb-Baseline}: Only the remaining time and reasoning time being used in the last round are provided as time cues.
\item \textbf{Static Bomb-Hint}: The system prompt includes a textual hint stating that reasoning consumes time, along with the number of tokens used in the previous reasoning step being provided in the state.
\item \textbf{Static Bomb-Hurry}: The user prompt includes an explicit urgency cue: \textit{“Hurry up! The bomb is going to explode soon.”}
\item \textbf{Static Bomb-Hint\&Hurry}: Combines both the system-level token-time hint and the user-level urgency signal.
\end{itemize}

All four variants share the same environment setup and differ only in how temporal cost is conveyed. The system prompt used for these settings is shown in~\Cref{fig:static_prompt}.
\input{Figures/s_static_prompt}

\paragraph{S3: Bomb Rush Hard.}
In this advanced setting, the bomb becomes a moving target, adding spatiotemporal uncertainty to the task. The agent must complete the mission under strict time constraints while adapting to different signal conditions. We consider two variants:

\begin{itemize}
\item \textbf{Moving Bomb Baseline (Passive Signal)}: The bomb moves randomly at each three step (slower than the agent) and continuously emits signals. The agent must reason under increased uncertainty about the bomb’s location while optimizing both navigation and timing.
The corresponding system prompt is shown in~\Cref{fig:moving_bomb_prompt}.
\input{Figures/s_moving_bomb_prompt}

\item \textbf{Moving Bomb with Active Detection}: The bomb still moves randomly, but no longer emits signals. To locate it, the agent must proactively choose to perform detection actions (sacrificing the chance to move), which consume valuable time. This variant tests the agent’s ability to balance information gathering with spatial progress under tight time budgets.
The corresponding system prompt is shown in~\Cref{fig:moving_bomb_wd_prompt}.
\input{Figures/s_moving_bomb_wd_prompt}
\end{itemize}



\section{Analysis on Step-wise Decision Accuracy}

Figure 7 further illustrates decision accuracy at different time progression stages for models under settings S1 and S2. This accuracy is calculated using the following formula:
$$ACC_t = \frac{\sum_{i=1}^{N_{t}} \delta{a}_{i}}{N_t}$$
where $\delta{a}_{i}$ equals 1 if action $a$ at step $i$ decreases the distance to the target, and 0 otherwise. Notably, distance here refers to the optimal path length determined by BFS search rather than Manhattan distance. We divided simulation steps into T buckets (T=15 in the figure) based on time progression (proportion of elapsed time to total time). $N_t$ represents the total number of actions in bucket $t$. For S1, where no time limit exists, progression is determined by the proportion of current steps to total steps. 

The figure reveals that although models experience accuracy degradation in later stages of S1, they maintain relatively high decision accuracy in early phases. We attribute the late-stage decline primarily to reasoning capacity deterioration caused by extended context windows. In S2, this decline manifests earlier, which we consider a potential side effect of time pressure on decision quality.
